A general method for computing thermal magnetic noise arising from thin conducting objects

Thermal motion of charge carriers in a conducting object causes magnetic field noise that interferes with sensitive measurements nearby the conductor. In this paper, we describe a method to compute the spectral properties of the thermal magnetic noise from arbitrarily-shaped thin conducting objects. We model divergence-free currents on a conducting surface using a stream function and calculate the magnetically independent noise-current modes in the quasi-static regime. We obtain the power spectral density of the thermal magnetic noise as well as its spatial correlations and frequency dependence. We describe a numerical implementation of the method; we model the conducting surface using a triangle mesh and discretize the stream function. The numerical magnetic noise computation agrees with analytical formulas. We provide the implementation as a part of the free and open-source software package bfieldtools.

==> noise_derivation.tex <==

To obtain the noise distribution for the magnetic field, we apply the equipartition theorem for our physical system. According to the theorem, in a thermal bath with temperature $T$ each independent degree of the system has $kT/2$ of energy on average. However, unless $\mathbf{M}$ and $\mathbf{R}$ are diagonal, the set of Langevin equations in \eqref{eq:5} are, coupled making the degrees of freedom dependent. To find the independent degrees of freedom, we must thus find a basis $\{ \vec{\kappa}_i(\vec{r}) \}$ where both the resistance and inductance matrices are diagonal.

As the matrices are symmetric positive-definite, the basis can be found by solving a generalized eigenvalue equation \cite{peeren2003stream, golub2012matrix}, i.e., finding a linear transformation $\mathbf{V}^T$ such that
\begin{equation} 
\label{eq:geneig}
\mathbf{R} \mathbf{V} = \mathbf{M} \mathbf{V} \boldsymbol{\Lambda} \Leftrightarrow
\left\{
	\begin{array}{ll}
		\mathbf{V}^T \mathbf{R} \mathbf{V} = \text{diag}(r_i, \dots, r_N) \\
		\mathbf{V}^T \mathbf{M} \mathbf{V} = \text{diag}(l_i, \dots, l_N),
	\end{array}
\right.
\end{equation}
where $\boldsymbol{\Lambda} = \text{diag}(\lambda_1 \dots \lambda_{N})$ is a diagonal matrix with $\lambda_i=r_i/l_i$. Application of the invertible but non-unitary transformation $\mathbf{V}^T$ to Eq. \eqref{eq:circuits} yields:
\begin{equation}
    -\frac{d}{dt} \mathbf{V}^T \mathbf{M} \mathbf{V} \mathbf{V}^{-1} \mathbf{j}(t) = \mathbf{V}^T \mathbf{R} \mathbf{V} \mathbf{V}^{-1} \mathbf{j}(t) +  \mathbf{V}^T \mathbf{e}(t).
\end{equation}
By defining $\tilde{\mathbf{j}}(t) = \mathbf{V}^{-1} \mathbf{j}(t)$ and $\tilde{\mathbf{e}}(t) = \mathbf{V}^{T} \mathbf{e}(t)$, we obtain decoupled Langevin equations
\begin{equation}\label{eq:rlcircuit}
    \frac{d}{dt} \tilde{j}_i(t) = -\lambda_i \tilde{j}_i(t) - \tilde{e}_i(t)/l_i\,.
\end{equation}
The generalized eigenvalues $\lambda_i = r_i/l_i = 1/\tau_i$ can now be interpreted as the reciprocals of the circuit time constants $\tau_i$. 

Modeling the emf as a white-noise process with spectral density $S_{\tilde{e}_i}$, the spectral density of $\tilde{j}_i$ can be solved from the decoupled circuit equation \cite{gillespie1996mathematics}
\begin{equation} \label{eq:jpsd}
    S_{\tilde{j}_i} (\omega) =  \frac{S_{\tilde{e}_i}}{r_i^2} \frac{1}{1 + ( \omega/\lambda_i)^2}\,.
\end{equation}
Integrating the spectral density over all frequencies gives the energy of the $i$th degree of freedom:
\begin{equation}
    E_i =  \frac{1}{2} l_i \frac{1}{2\pi}\int_{0}^{\infty} S_{\tilde{j}_i} (\omega) d\omega = \frac{1}{2} l_i \frac{S_{\tilde{e}_i}}{4 r_i^2}\lambda_i=\frac{S_{\tilde{e}_i}}{8 r_i}\,.
\end{equation}
On the other hand, according to the equipartition theorem, the average  equals to $E_i = \frac{1}{2} k T$, which is then equivalent to
\begin{equation}
    S_{\tilde{e}_i} (\omega) = 4 kTr_i\,,
\end{equation}
where $r_i$ can be associated with the average power dissipation of the mode $i$, i.e., $P_i = r_i \langle \tilde{j}_i(t)^2 \rangle$.


Thermal noise currents are driven by the Johnson emf that is proportional to a zero-mean temporal Gaussian white noise process $\Gamma(t)$ \cite{gillespie1996mathematics}. To obtain the spatial Johnson noise current modes and their variance, we decouple the circuit equations \eqref{eq:circuits} by finding a basis $\{ \vec{\kappa}_i(\vec{r}) \}$ where both the resistance and inductance matrices are diagonal,  i.e., $\tilde{R}_{ij} = r_{ij} \delta_{ij}$ and $\tilde{M}_{ij} = l_{ij} \delta_{ij}$, where $r_{i} = r_{ii}$ and $l_{i}=l_{ii}$ are the resistance and self-inductance of the decoupled circuit $\vec{\kappa}_i$, respectively.
%\begin{align}
%    \tilde{R}_{ij} &= \int_S \frac{1}{\sigma(\vec{r}) d(\vec{r})} \vec{\kappa}_i(\vec{r}) \cdot  \vec{\kappa}_j(\vec{r}) dS = r_{ij} \delta_{ij} \label{eq:diagR} \\
%    \tilde{M}_{ij} &= \frac{\mu_0}{4\pi}\int_S \int_S \frac{\vec{\kappa}_i(\vec{r}) \cdot  \vec{\kappa}_j(\vec{r}\,')}{|\rr|} dS dS' = l_{ij} \delta_{ij}, \label{eq:diagM}
%\end{align}
%where $r_{i} = r_{ii}$ and $l_{i}=l_{ii}$ are the resistance and self-inductance of the decoupled circuit $\vec{\kappa}_i$, respectively.
We note that both $\mathbf{M}$ and $\mathbf{R}$ are Hermitian and positive definite for an ordinary conductor \cite{zevenhoven2014conductive}. In the following, we will assume that they are also real. The decoupled circuits can be found by solving a generalized eigenvalue equation \cite{peeren2003stream,golub2012matrix}, i.e., finding a linear transformation $\mathbf{V}^T$ for which 
\begin{equation} 
\label{eq:geneig}
\mathbf{R} \mathbf{V} = \mathbf{M} \mathbf{V} \boldsymbol{\Lambda} \Leftrightarrow
\left\{
	\begin{array}{ll}
		\mathbf{V}^T \mathbf{R} \mathbf{V} = \text{diag}(r_i, \dots, r_N) \\
		\mathbf{V}^T \mathbf{M} \mathbf{V} = \text{diag}(l_i, \dots, l_N),
	\end{array}
\right.
\end{equation}
where $\boldsymbol{\Lambda} = \text{diag}(\lambda_1 \dots \lambda_{N})$ is a diagonal matrix with $\lambda_i = r_i/l_i = 1/\tau_i$ as the reciprocals of the circuit time constants $\tau_i$. We also assumed that the magnetic field due to the Johnson current is presented in sufficient accuracy with $N$ modes.

%, i.e., $\boldsymbol{\Lambda} = \text{diag}(r_i, \dots, r_N) [\text{diag}(l_i, \dots, l_N)]^{-1}$.

Application of the invertible but non-unitary transformation $\mathbf{V}^T$ to Eq. \eqref{eq:circuits} yields:
\begin{equation}
    -\frac{d}{dt} \mathbf{V}^T \mathbf{M} \mathbf{V} \mathbf{V}^{-1} \mathbf{j}(t) = \mathbf{V}^T \mathbf{R} \mathbf{V} \mathbf{V}^{-1} \mathbf{j}(t) +  \mathbf{V}^T \mathbf{e}(t).
\end{equation}
By defining $\tilde{\mathbf{j}}(t) = \mathbf{V}^{-1} \mathbf{j}(t)$ and $\tilde{\mathbf{e}}(t) = \mathbf{V}^{T} \mathbf{e}(t)$, we obtain the decoupled circuit (Langevin) equations
\begin{equation}\label{eq:rlcircuit}
    -l_i \frac{d}{dt} \tilde{j}_i(t) = r_i \tilde{j}_i(t) + \tilde{e}_i(t).
\end{equation}
For the decoupled circuits, the average power dissipation \eqref{eq:powdiss} as well as magnetic energy \eqref{eq:magenergy} are diagonal
\begin{align}
    P_i &= r_i \langle \tilde{j}_i(t)^2 \rangle \\
    E_i &= \frac{1}{2} l_i \langle \tilde{j}_i(t)^2 \rangle .
\end{align}

The variance of the Johnson emf coupled to the magnetically independent circuits can be derived using the equipartition theorem, which states that the equilibrium circuit currents at temperature $T$ have a magnetic energy of \cite{gillespie1996mathematics}
\begin{equation}
    E_i = \frac{1}{2} l_i \langle \tilde{j}_i(t)^2 \rangle = \frac{1}{2}k T,
\end{equation}
where $k$ is the Boltzmann constant. Using this requirement for the circuit currents and considering the properties of fully relaxed Ornstein--Uhlenbeck process (see Ref. \cite{gillespie1996mathematics}), the fluctuation--dissipation formula for the white noise Johnson emf can be derived as
\begin{equation}
    \tilde{e}_i(t) = (2kT r_i)^{1/2} \Gamma(t),
\end{equation}
whose power spectral density (PSD) is given by the Nyquist formula \cite{gillespie1996mathematics}
\begin{equation}
    S_{\tilde{e}_i} (\omega) = 4 kTr_i.
\end{equation}
The PSD of the noise current can be solved from the decoupled circuit equation \eqref{eq:rlcircuit} \cite{gillespie1996mathematics}
\begin{equation} \label{eq:jpsd}
    S_{\tilde{j}_i} (\omega) = \frac{4 kT}{r_i} \frac{1}{1 + ( l_i \omega/r_i)^2}.
\end{equation}
The PSD has the form of white noise filtered by a first-order low-pass filter with a cutoff frequency equal to the reciprocal of the circuit time constant $r_i/l_i$.


\noindent We assume a thin (compared to the observation distance) conducting surface $S$ with conductivity $\sigma(\vec{r})$ and thickness $d(\vec{r})$. We also assume that the current density is divergence-free ($\nabla \cdot \vec{J} = 0$).  The divergence-free surface current density on $S$ can be expressed using a stream function $\Psi$ (units A/m) as \cite{zevenhoven2014conductive}
\begin{equation}
\label{eq:sfrepres}
    \vec{J}(\vec{r}, t) = \nabla_{\|} \Psi(\vec r, t)  \times  \n(\vec r),
\end{equation}
where $\n$ is the unit surface normal and $\nabla_{\|}$ is the tangential gradient on the surface. We further express the stream function in a basis $\Psi(\vec r,t) = \sum_i s_i(t) \psi_i(\vec{r})$ with coefficients $s_i(t)$ (units A) giving
\begin{equation}
\label{eq:krepres}
    \vec{J}(\vec{r}, t) = \sum_i s_i(t) \nabla_{\|} \psi_i(\vec{r}) \times  \n(\vec r) = \sum_i s_i(t) \vec{k}_i(\vec{r}),
\end{equation}
where $\vec{k}_i(\vec{r}) = \nabla_{\|} \psi_i(\vec{r}) \times  \n(\vec r)$. The current density is then given as a linear combination of current-density patterns $\vec{k}_i(\vec{r})$ weighted by time-dependent coefficients representing their currents.

 The current density is then given as a linear combination of current-density patterns $\vec{k}_i(\vec{r})$ weighted by time-dependent coefficients representing their currents.
 
 The average resistive power dissipation between the modes $i$ and $j$ is
\begin{align}
\label{eq:powdiss}
    P_{ij} &= \langle  j_i(t) j_j(t) R_{ij} \rangle \nonumber \\
    &=  \langle j_i(t) j_j(t) \rangle \int_S \frac{1}{\sigma(\vec{r}) d(\vec{r})} \vec{k}_i(\vec{r}) \cdot  \vec{k}_j(\vec{r}) dS,
\end{align}
where the brackets $\langle \cdot \rangle$ denote expectation and $R_{ij}$ is the mutual resistance between the patterns \cite{zevenhoven2014conductive}. The average inductive energy between the patterns is given in turn by the mutual inductance $M_{ij}$ \cite{zevenhoven2014conductive}
\begin{align}
\label{eq:magenergy}
    E_{ij} &= \frac{1}{2} \langle j_i(t) j_j(t) M_{ij} \rangle \nonumber\\
    &= \frac{1}{2} \langle j_i(t) j_j(t) \rangle \frac{\mu_0}{4\pi} \int_S \int_S \frac{\vec{k}_i(\vec{r}) \cdot  \vec{k}_j(\vec{r}\,')}{|\rr|} dS dS'.
\end{align}

The currents of the patterns can be described by coupled RL-circuit equations (\cite{zevenhoven2014conductive}; \ref{app:circuiteq})
\begin{equation}
\label{eq:circuits}
    -\mathbf{M} \frac{d}{dt} \mathbf{j}(t) = \mathbf{R} \mathbf{j}(t) +  \mathbf{e}(t),
\end{equation}
where $\mathbf{j}[i](t) = j_i(t)$ is the current of the $i$th pattern, $\mathbf{M}[i,j] = M_{ij}$ and $\mathbf{R}[i,j] = R_{ij}$ are the mutual inductance and resistance matrices defined above and $\mathbf{e}(t)$ is the electromotive force (emf) coupled to the pattern. Equation \eqref{eq:circuits} allows to draw an analogy between the stream-function representations of the current patterns \eqref{eq:krepres} and coupled RL circuits. Leveraging this analogy, from now on we will refer to $\vec{k}_i(\vec{r})$ and $j_i(t)$ as the $i$th circuit and its current, respectively. We note that the normalization of the stream function affects the physical interpretation of $\mathbf{M}$ and $\mathbf{R}$ \cite{zevenhoven2014conductive}.

By defining $\tilde{\mathbf{j}}(t) = \mathbf{V}^{-1} \mathbf{j}(t)$ and $\tilde{\mathbf{e}}(t) = \mathbf{V}^{T} \mathbf{e}(t)$, we obtain a set of decoupled Langevin equations
\begin{equation}\label{eq:rlcircuit}
    \frac{d}{dt} \tilde{j}_i(t) = -\lambda_i \tilde{j}_i(t) - \tilde{e}_i(t)/l_i\,.
\end{equation}
The equations can be interpreted to represent RL-circuits with time constants $\tau_i = l_i/r_i = 1 / \lambda_i$ driven by the Johnson emf $\tilde{e}_i(t)$. These circuits effectively constitute the independent degrees of freedom of the system.
